Coding Agents Are Zero-Shot Coordinators

Zero-shot coordination (ZSC) requires independently developed agents to cooperate with unseen partners, including humans. Current methods make progress towards this goal, but rely on restrictive assumptions. On benchmarks such as Overcooked V2 and Yokai, they are either difficult to apply or, even when applicable, perform poorly. This led to an expectation that further progress requires algorithmic innovation. Surprisingly, we find that these challenges are addressed with an increase in the general capability of large language models (LLMs). Coding agents, which pair an LLM with an off-the-shelf coding harness, achieve state-of-the-art results on both benchmarks by generating policies as code and refining them using only self-play feedback. Further, ZSC aims to enable coordination with humans, yet its standard formulation overlooks settings where humans pre-agree on conventions without joint training (e.g, Hanabi). Towards this, we extend ZSC by providing agents with shared conventions in natural language. In Hanabi, given conventions used by human players, coding agents outperform baselines in cross-play with the Will-Hanabi bot. Finally, we use the generated policies to guide convention selection during self-play, achieving the highest cross-play with both the Will-Hanabi and the AH2AC2 bots trained on human gameplay logs. Code is available at https://shshnkreddy.github.io/coding-agent-zsc.

==> Figures/learning_algorithm_diagram.tex <==
% Vector artwork shared by the paper figure and its standalone export.
\begingroup%
\definecolor{agent}{HTML}{385673}%
\definecolor{env}{HTML}{008577}%
\definecolor{ink}{HTML}{30343B}%
\definecolor{secondary}{HTML}{626B75}%
\definecolor{rule}{HTML}{A8ADB4}%
\definecolor{agentfill}{HTML}{EDF2F7}%
\definecolor{envfill}{HTML}{E0F5F0}%
\begin{tikzpicture}[x=1pt,y=1pt,
 every node/.style={inner sep=0pt,outer sep=0pt,text=ink,font=\fontsize{9}{11}\fontencoding{T1}\fontfamily{phv}\selectfont},
 heading/.style={font=\fontsize{10}{12}\fontencoding{T1}\fontfamily{phv}\bfseries\selectfont},
 note/.style={text=secondary,font=\fontsize{8}{10}\fontencoding{T1}\fontfamily{phv}\selectfont},
 frame/.style={line width=.55pt,rounded corners=2pt},
 flow/.style={->,>=stealth,draw=secondary,line width=.7pt},
 branch/.style={draw=rule,line width=.45pt},
 zoom/.style={draw=rule,line width=.45pt,dash pattern=on 2.5pt off 2.5pt},
 file/.style={anchor=base west,font=\fontsize{9.8}{11}\fontencoding{T1}\fontfamily{pcr}\selectfont},
 directory/.style={file,text=env,font=\fontsize{9.8}{11}\fontencoding{T1}\fontfamily{pcr}\bfseries\selectfont},
 tag/.style={anchor=base west,text=secondary,font=\fontsize{8.2}{10}\fontencoding{T1}\fontfamily{pcr}\selectfont}]
 % Let TikZ fit its bounds to the artwork, including stroke widths.

 % Magnification guide, distinct from the environment frame and tool arrows.
 \draw[zoom] (258,-51) -- (280,-51) -- (291,-10);
 \draw[zoom] (258,-77) -- (280,-77) -- (291,-170);
 \draw[branch] (297,-10) -- (291,-10) -- (291,-170) -- (297,-170);

 \begin{scope}[yshift=14pt]
 \draw[frame,draw=agent,line width=1pt,fill=white] (5,-59) rectangle (94,-118);
 \node[heading,text=agent,anchor=base,inner ysep=0.5pt] at (49.5,-50) {Coding agent $\mathcal{C}$};
 \draw[frame,draw=agent,fill=agentfill] (10,-83) rectangle (89,-113);
 \node[heading,text=agent] at (49.5,-93) {\acs*{llm} $L$};
 \node[note] at (49.5,-105) {Frozen parameters};
 \node at (49.5,-69) {Harness $\mathcal{H}$};

 \draw[frame,draw=env] (169,-60) rectangle (263,-156);
 \node[heading,text=env,anchor=base,inner ysep=0.5pt] at (216,-50) {Environment $\mathcal{E}$};
 \draw[frame,draw=env,fill=envfill] (174,-65) rectangle (258,-91);
 \node[heading,text=env] at (216,-78) {Workspace};
 \draw[flow] (94,-73) -- (174,-73);
 \node[note,align=center,fill=white] at (132,-59) {Tool calls\\(Read, Edit, etc.)};
 \draw[flow] (174,-85) -- (94,-85);
 \node[note,fill=white] at (132,-79) {Tool call outputs};

 \draw[frame,draw=env,fill=white] (174,-129) rectangle (258,-151);
 \node[heading,text=env] at (216,-140) {Policy runtime};
 \draw[flow] (196,-91) -- (196,-129);
 \node[note,anchor=east] at (191,-110) {Code};
 \draw[flow] (224,-129) -- (224,-91);
 \node[note,anchor=west,align=left] at (230,-110) {Returns,\\traces,\\errors};
 \draw[flow] (53,-118) -- (53,-140) -- (174,-140);
 \node[note,fill=white] at (128,-132) {Evaluate};
 \end{scope}

 % Each successive column is one directory depth, not a flow of execution.
 \begin{scope}[yshift=4pt]
 \node[directory] at (303,-104) {task/};
 \draw[branch] (334,-101) -- (338,-101);
 \draw[branch] (338,-17) -- (338,-151);
 \foreach \y in {17,43,101,151} \draw[branch] (338,-\y) -- (345,-\y);

 \node[file] at (349,-20) {AGENTS.md};
 \node[directory] at (349,-46) {bin/};
 \node[tag] at (349,-58) {\# read only};
 \node[directory] at (349,-104) {context/};
 \node[tag] at (349,-116) {\# read only};
 \node[directory] at (349,-154) {workspace/};
 \node[tag] at (349,-166) {\# editable};

 \draw[branch] (378,-43) -- (420,-43);
 \draw[branch] (420,-31) -- (420,-55);
 \foreach \y in {31,43,55} \draw[branch] (420,-\y) -- (426,-\y);
 \node[file] at (429,-34) {policy-eval};
 \node[file] at (429,-46) {policy-ledger};
 \node[file] at (429,-58) {policy-lifetime};

 % Reduce the gap after bin/ by 4pt, keeping each group internally aligned.
 \begin{scope}[yshift=4pt]
 \draw[branch] (402,-105) -- (420,-105);
 \draw[branch] (420,-75) -- (420,-135);
 \foreach \y in {75,87,99,111,123,135} \draw[branch] (420,-\y) -- (426,-\y);
 \node[file] at (429,-78) {task\_spec.md};
 \node[file] at (429,-90) {policy\_api.md};
 \node[file] at (429,-102) {starting\_policy.py};
 \node[file] at (429,-114) {rollout\_api.py};
 \node[directory] at (429,-126) {environment/};
 \node[directory] at (429,-138) {conventions/};
 \end{scope}

 % Tighten the gap after context/ while retaining separation between groups.
 \begin{scope}[yshift=10pt]
 \draw[branch] (412,-161) -- (420,-161);
 \draw[branch] (420,-155) -- (420,-167);
 \foreach \y in {155,167} \draw[branch] (420,-\y) -- (426,-\y);
 \node[file] at (429,-158) {policy.py};
 \node[file] at (429,-170) {rollouts.py};
 % \node[file] at (445,-182) {experiment\_ledger.md};
 % \node[tag] at (550,-182) {\# tool-managed};
 \end{scope}
 \end{scope}
\end{tikzpicture}%
\endgroup%

